Simultaneously Reconciled Quantile Forecasting of Hierarchically Related Time Series

Many real-life applications involve simultaneously forecasting multiple time series that are hierarchically related via aggregation or disaggregation operations. For instance, commercial organizations often want to forecast inventories simultaneously at store, city, and state levels for resource planning purposes. In such applications, it is important that the forecasts, in addition to being reasonably accurate, are also consistent w.r.t one another. Although forecasting such hierarchical time series has been pursued by economists and data scientists, the current state-of-the-art models use strong assumptions, e.g., all forecasts being unbiased estimates, noise distribution being Gaussian. Besides, state-of-the-art models have not harnessed the power of modern nonlinear models, especially ones based on deep learning. In this paper, we propose using a flexible nonlinear model that optimizes quantile regression loss coupled with suitable regularization terms to maintain the consistency of forecasts across hierarchies. The theoretical framework introduced herein can be applied to any forecasting model with an underlying differentiable loss function. A proof of optimality of our proposed method is also provided. Simulation studies over a range of datasets highlight the efficacy of our approach.

==> SHARQ-AISTATS21 (Version 7138)/tex/analysis.tex <==
\newcommand\Item[1][]{%
  \ifx\relax#1\relax  \item \else \item[#1] \fi
  \abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}
  
\section{Statistical Analysis of SHARQ} \label{theory}
In this section, we theoretically demonstrate the advantages of SHARQ. We begin by showing the optimality of our formulation (\ref{contstrained_loss}) in contrast to post-inference based methods, which solves the matrix $P$ for $\ty_T(h) = SP\hy_T(h)$. We emphasize our advantage in balancing coherency requirements and forecasting accuracy. We then present some desirable statistical properties of SHARQ. 

\begin{thm}\textbf{(Global Optimum)} \label{thm:loss}
For $L_c \in C^1$, for an arbitrary parameterized smooth regressor model asymptotically,
\begin{align} 
&\L_c (g_i (X_m^i, \theta^{\star}_i), ~ Y_m^i, ~~ g_k (X_m^k, \theta^{\star}_k)) \nonumber \\
&\le \L_c (g_i (X_m^i, \theta^{recon}_i), ~ Y_m^i, ~~ g_k (X_m^k, \theta^{recon}_k))
\end{align}
where $\theta^{\star}$, $\theta^{recon}$ are the parameters for SHARQ, and post inference reconciled solution, respectively. 
\end{thm}

\begin{proof}
By definition, SHARQ directly minimize Eq.(\ref{contstrained_loss}),
\begin{equation}
    \theta^{\star} = \arg \underset{\theta}{\min} ~\L_c (g_i (X_m^i, \theta_i), ~ Y_m^i, ~~ g_k (X_m^k, \theta_k)),
\end{equation}
where $\theta = \{\theta_i, \theta_k\}$. 
\end{proof}
Since \citet{ben2019regularized, hyndman2011optimal, hyndman2016fast, wickramasuriya2015forecasting} are performing the reconciliation as a post-processing step, those solutions are bound to be sub-optimal in comparison with $\theta^{\star}$.
\begin{pro}\textbf{(Hard Constraint)} \label{thm:stats}
For post-inference based methods, $P \hat{y}_T (h)$ is the bottom level reconciled forecast. In other words, it requires that 
\begin{equation}
    g_i (X_m^i, \theta^{\star}_i) = \sum_{e_{i, k} \in E} g_k (X_m^k, \theta^{recon}_k).
    \label{equ:stats_pro}
\end{equation}
Had we only considered the point forecast reconciliation, i.e. $\E[g_i (X_m^i, \theta^{\star}_i)] = \sum_{e_{i, k} \in E} \E[g_k (X_m^k, \theta^{recon}_k)],$ the post inference processing still might have worked. However, due to the probabilistic nature of the variables $g_i (X_m^i, \theta^{\star}_i) = \E[g_i (X_m^i, \theta^{\star}_i)] + \varepsilon_i$, where $\varepsilon_i$ is the observation noise, reconciling the mean won't suffice.
\end{pro}
\paragraph{Remark}  To satisfy Eq.(\ref{equ:stats_pro}), it is required that $\varepsilon_i = \sum_{e_{i, k} \in E} \varepsilon_k$, which is not a realistic property to be satisfied in real-life problems. Intuitively, when a reconciliation matrix $P$ is applied, the original, unbiased base forecasts with variation are ``forced'' to be summed up. However, our method does not impose this hard constraint, leading to different properties.

\begin{figure*}[t]
\centering
{
\setlength{\tabcolsep}{1pt} 
\renewcommand{\arraystretch}{1} 
\begin{tabu}{ccc}
\hspace{-0.45em}
\includegraphics[width=.33\textwidth]{images/log_sine.png}&
\hspace{-0.45em}
\includegraphics[width=.33\textwidth]{images/gamma_piecewise.png}&
\hspace{-0.45em}
\includegraphics[width=.33\textwidth]{images/Gaussian_piecewise.png} \\
\hspace{-0.45em} (a) Log-normal error & \hspace{-0.45em} (b) Gamma error & \hspace{-0.45em} (c) Gaussian error \\
\end{tabu}
}
\caption{Forecasting results of simulated sequential data under different error distributions. The original function of (a) is sinusoidal with varying frequency; (b) and (c) are discontinuous step functions. Note that our baseline forecasts in (b) and (c) are overconfident \citep{lakshminarayanan2017simple, li2020improving} and their prediction intervals are too small to be shown.}
\label{fig:sim_plot}
\end{figure*}

\usetikzlibrary{fit,backgrounds} % <-added
\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes,arrows}

\tikzstyle{rect} = [draw, rectangle, fill=white!20, text width=2em, text centered, minimum height=2em]
\tikzstyle{longrect} = [draw, rectangle, fill=white!20, text width=6em, text centered, minimum height=2em]
\tikzstyle{circ} = [draw, circle, fill=white!20, radius=2.6, minimum size=.8cm, inner sep=0pt]
\tikzstyle{line} = [draw, -latex']

\begin{table*}[t]
\centering
\renewcommand\arraystretch{1.7}
\begin{minipage}{.41\textwidth}
\scalebox{0.77}{
\begin{tabular}{c|c|c|c|c}
\hlinewd{1.3pt}
\multicolumn{2}{c}{ Error distribution } & Log-normal & Gamma & Gaussian \\ \hline
\multirow{2}{*}{ MAPE } & Quantile & \textbf{32.72} & \textbf{62.20} & \textbf{70.29} \\
& Baseline & 49.88 & 73.69 & 73.36 \\ \hline
\multirow{2}{*}{ LR } & Quantile & \textbf{0.2218} & \textbf{0.5649} & \textbf{0.8634} \\
& Baseline & 0.5661 & 0.7489 & 1.025 \\
\hlinewd{1.3pt}
\end{tabular}}
\end{minipage}
\begin{minipage}{.57\textwidth}
\centering
    \begin{tikzpicture}[node distance = 1.2cm,auto]
    \node [rect, rounded corners, label={[font=\small\sffamily,name=label1]above:{Forecasting model}}] (step1) {$h_{t-2}$};
    \node [rect, right of=step1, rounded corners] (step2) {$h_{t-1}$};
    \node [rect, right of=step2, rounded corners] (step4) {$h_t$};
    \node [rect, right of=step4, rounded corners] (step8) {$o_t$};
    \node [circ, below of=step1] (step5) {$x_{t-2}$};
    \node [circ, below of=step2] (step6) {$x_{t-1}$};
    \node [circ, below of=step4] (step7) {$x_t$};
    \node [longrect, above right = 0.2cm and 0.3cm of step8] (step9) {dense layer 1};
    \node [longrect, below right = 0.2cm and 0.3cm of step8] (step10) {dense layer 3};
    \node [longrect, right =0.25cm of step8] (step12) {dense layer 2};
    \node [circ, right =0.2cm of step12] (step11) {$\hat{y}^{\tau}_{t+1}$};
    \path [line] (step1) -- (step2);
    \path [line] (step2) -- (step4);
    \path [line] (step5) -- (step1);
    \path [line] (step6) -- (step2);
    \path [line] (step7) -- (step4);
    \path [line] (step4) -- (step8);
    \path [line, rounded corners] (step8) |- (step9);
    \path [line, rounded corners] (step8) |- (step10);
    \path [line, rounded corners] (step9) -| (step11);
    \path [line, rounded corners] (step10) -| (step11);
    \path [line] (step8) -- (step12);
    \path [line] (step12) -- (step11);
    \begin{scope}[on background layer]
    \node[draw,dashed,black,rounded corners,fill=gray!50,fit=(step1) (step2) (step4) (step5) (step6) (step7) (label1)]{};
    \end{scope}
    \end{tikzpicture}
\end{minipage}
\caption{Left: Quantitative results for simulation experiments. We use Mean Absolute Percentage Error (MAPE) \citep{makridakis2000m3} to measure forecasting accuracy and Likelihood Ratio (LR) to evaluate uncertainty intervals. Right: A schematic of the multi-quantile forecaster used for simulation.}
\label{tab:sim_res}
\end{table*}


\begin{pro}\textbf{(Unbiasedness Property)}
Consider a hierarchical structure with $n$ nodes where the first $\kappa$ nodes belong to aggregation levels, assume that the bottom level forecasting is unbiased:
\begin{equation}
    \E [g_k (X_m^k, \theta_k)] = Y_m^k, \quad k = \kappa + 1,..., n
\end{equation}
and the bottom level forecasting models are well optimized:
\begin{equation}
     \mathrm{Var}\left(\|g_k (X_m^k, \theta_k) - Y_m^k\|\right) = \epsilon, \quad
     \epsilon = \mathcal{O}(\frac{1}{m}).
\end{equation}
Then we have that
\begin{align*}
    \E[g_i (X_m^i, \theta_i)] & = \E[\sum_{e_{i, k} \in E} g_k (X_m^k, \theta_k)] \nonumber \\
    & = \sum_{e_{i, k} \in E} \E[g_k (X_m^k, \theta_k)] \nonumber \\
    & = Y_m^i, \quad i = 1, ..., \kappa
\end{align*}
\end{pro}
Therefore, we claim that given the unbiased base forecast at the most disaggregated level, as well as well-specified models, our method can provide unbiased estimation at all aggregation levels.
\begin{pro}\textbf{(Variance Reduction)}
Assume we are minimizing a quadratic loss function using our formulation, where
\begin{align*}
& L_c (g_i (X_m^i, \theta_i), Y_m^i, g_k (X_m^k, \theta_k)) = \|g_i (X_m^i, \theta_i) - Y_m^i\|^2 \nonumber \\
& + \lambda_i  \parallel g_i (X_m^i, \theta_i) - \sum_{e_{i, k} \in E} \left ( e_{i, k} ~g_k (X_m^k, \theta_k)  \right ) \parallel^2.
\end{align*}
By solving the quadratic objective, we get
\begin{equation}
    g_i (X_m^i, \theta_i) = \frac{Y_m^i + \lambda_i \sum_{e_{i, k} \in E} e_{i, k} ~g_k (X_m^k, \theta_k)}{\lambda_i + 1}.
\end{equation}
Note that if we fit linear models that generalize in the bottom level, we have $\mathrm{Var} (\sum_{e_{i, k} \in E} e_{i, k} ~g_k (X_m^k, \theta_k)) = \mathcal{O}(\frac{1}{m})$ (for other models, the variance should be at least in a smaller scale than $\mathcal{O}(1)$, which is the variance of observed samples). Therefore, by alternating $\lambda_i$:
\begin{itemize}
    \item $\mathrm{Var}(g_i (X_m^i, \theta_i)) = \mathrm{Var}(Y_m^i) = \mathcal{O}(1), \mathrm{when} ~\lambda_i \rightarrow 0$.
    \Item
    \begin{align}\hspace{-1.75em}
    	\mathrm{Var}(g_i(X_m^i, \theta_i)) & = \mathrm{Var}(\sum_{e_{i, k} \in E} e_{i, k} ~ g_k (X_m^k, \theta_k)) \nonumber \\
    	& = \mathcal{O}(\frac{1}{m}), \mathrm{when} ~ \lambda_i \rightarrow \infty.
    \end{align}
\end{itemize}
\end{pro}

This tells us that by alternating the coefficient $\lambda_i$, the amount of estimator variance at higher aggregation levels can be controlled. If lower-level models are accurate, then we can improve the higher-level models by this method. Instead of adding a hard coherency requirement like the post-inference methods, SHARQ provides more flexibility for controlling the variations.

==> SHARQ-AISTATS21 (Version 7138)/tex/conclusion.tex <==
\section{Conclusion} \label{conclusion}
This paper has proposed a distributed optimization framework to generate probabilistic forecasts for a set of time series subject to hierarchical constraints. In our approach, the forecasting model is trained in a bottom-up fashion. At any stage, the model training involves simultaneously updating model parameters at two adjacent levels while maintaining the coherency constraints. This enables manageable information exchange at different levels of data aggregation. Our framework can incorporate any forecasting model and the non-parametric quantile loss function to generate accurate and coherent forecasts with pre-specified confidence levels. We have analytically demonstrated that by training the model with our modified objective function, the variance of time series data at higher aggregation levels can be reduced. We also compared our method empirically with the state-of-the-art hierarchical forecasting methods with cutting-edge base forecasters. The results show that our method produces relatively robust with accurate and coherent forecasts. Our proposed method reduces the inference complexity compared to the state-of-the-art algorithms, which perform a computationally expensive matrix inversion operation during the inference to achieve the reconciliation. 

As for future work, we plan to extend our method to multi-variate time series to be forecast at different time granularities while obeying hierarchical relationships. Besides, we also plan to investigate incorporating exogenous variables and related metadata. 

\textbf{Acknowledgements} \\
% \newline
This work is supported by Intuit Inc. The authors would like to thank all reviewers for their constructive feedback and Tongzheng Ren for helpful discussion.
%\section{Boarder Impact}
%
%Forecasting Hierarchical Time Series has many several applications, including financial forecasting, inventory prediction, industrial management, cloud resources optimization, psephology related forecasts and many more. For example in corporate financial forecasting, total profit, revenue, expense, assets, equities, liabilities etc are to be predicted where these individual categories form a hierarchical structure as well as there are other accounting related constraints which can be incorporated into the hierarchical framework. Also, often companies want to forecast net revenue and expenses for major business account which form further levels of hierarchies. For corporate short term and long term planning purposes the forecasts are to be generated at different temporal aggregation granularity levels like daily, weekly, monthly, quarterly and so on. Retail chains and global ecommerce companies forecast demand for different items at store level, city level, state and country levels. The time series data is often sparse for the bottom level of the hierarchy (e.g. store level for each product). An inaccurate prediction can lead to millions of dollars worth financial loss to the company. Utilizing the hierarchical structure forecasts can be improved as well as consistency of the forecasts can be maintained across the hierarchy, which can lead to enormous savings. The electoral opinion pole forecasts are made also at country, state, county or city levels. Developing accurate and consistent probabilistic forecasts for hierarchical time series will be greatly beneficial to several industrial applications.  

==> SHARQ-AISTATS21 (Version 7138)/tex/experiments.tex <==
\section{Experimental Results} \label{experimental_results}
In this section, we validate the performance of SHARQ on multiple hierarchical time series datasets with different properties and use cases. The experiments are conducted on both simulated and real-world data. Results demonstrate that SHARQ can generate coherent and accurate forecasts and well-capture the prediction uncertainty at any specified level.

\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.2}
\caption{Performance measured by MAPE \citep{makridakis2000m3} on Australian Labour (755 time series), and M5 competition (42840 time series), lower values are better. Level 1 is the top aggregation level, and 4 is the bottom level.}
\scalebox{0.7}{
\begin{tabular}{c|cccc|cccc|cccc|cccc}
\hlinewd{1.5pt}
Algorithm & \multicolumn{4}{c}{ RNN } & \multicolumn{4}{c}{ Autoregressive } & \multicolumn{4}{c}{ LST-Skip } & \multicolumn{4}{c}{ N-Beats } \\
\hline
\multirow{2}{*}{ Reconciliation } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } \\ \hhline{|~|----|----|----|----|}
& 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 \\ \hline
BU & 15.23 & 15.88 & 19.41 & \textbf{17.96} & 19.29 & 20.14 & 21.09 & 22.13 & 16.13 & 17.59 & 16.88 & \textbf{17.17} & 14.23 & 14.75 & 15.67 & \textbf{15.84} \\
Base & 12.89 & 14.26 & 16.96 & \textbf{17.96} & \textbf{17.59} & 19.86 & 20.98 & 22.13 & 14.99 & 12.31 & \textbf{15.12} & \textbf{17.17} & 12.18 & 13.32 & \textbf{14.32} & \textbf{15.84} \\
MinT-sam & 14.98 & 15.94 & 17.79 & 19.23 & 18.82 & 19.98 & 21.59 & 22.26 & 15.12 & 14.41 & 16.42 & 18.62 & 13.11 & 14.63 & 14.86 & 15.96 \\
MinT-shr & 14.46 & 15.43 & 16.94 & 18.75 & 18.54 & 19.98 & 21.22 & 22.01 & 15.06 & 13.89 & 16.31 & 17.56 & 12.76 & 14.41 & 14.77 & 15.87 \\
MinT-ols & 15.01 & 15.96 & 18.75 & 19.21 & 19.14 & 20.02 & 21.74 & 22.34 & 15.12 & 14.41 & 16.41 & 18.74 & 13.29 & 14.49 & 14.85 & 16.83 \\
ERM & 14.73 & 16.62 & 19.51 & 20.13 & 17.89 & 20.11 & 20.33 & \textbf{21.93} & 16.61 & 16.84 & 18.75 & 19.21 & 14.52 & 15.26 & 17.02 & 17.29 \\
SHARQ & \textbf{12.55} & \textbf{13.21} & \textbf{16.01} & \textbf{17.96} & 17.65 & \textbf{19.72} & \textbf{20.01} & 22.13 & \textbf{11.97} & \textbf{12.24} & 15.64 & \textbf{17.17} & \textbf{11.86} & \textbf{12.35} & 14.53 & \textbf{15.84} \\ \hhline{|=|====|====|====|====|}
BU & 11.42 & 12.04 & 12.32 & \textbf{11.72} & 12.77 & 14.59 & 16.11 & \textbf{16.56} & 10.11 & 12.69 & 10.78 & \textbf{10.94} & 11.01 & 11.05 & 12.43 & \textbf{11.34} \\
Base & 10.63 & 10.15 & 11.23 & \textbf{11.72} & 11.64 & 13.91 & 15.67 & \textbf{16.56} & 8.96 & 11.38 & 10.59 & \textbf{10.94} & 9.64 & 9.88 & 11.11 & \textbf{11.34} \\
MinT-sam & 11.25 & 11.67 & 11.87 & 12.99 & 12.34 & 14.09 & 15.97 & 17.54 & 9.64 & 12.31 & 11.02 & 11.01 & 9.97 & 10.82 & 11.89 & 12.77 \\
MinT-shr & 10.76 & 11.03 & 11.49 & 12.81 & 11.92 & 13.85 & 15.76 & 17.33 & 9.19 & 11.97 & 10.71 & 10.99 & 9.78 & 10.69 & 11.56 & 12.63 \\
MinT-ols & 11.75 & 11.56 & 12.06 & 13.05 & 12.32 & 14.21 & 15.97 & 17.56 & 9.63 & 12.54 & 10.98 & 11.02 & 10.41 & 11.01 & 12.02 & 12.71 \\
ERM & 11.86 & 12.01 & 12.42 & 13.54 & 12.61 & 14.02 & \textbf{15.41} & 17.14 & 10.35 & 13.01 & 13.15 & 13.56 & 10.44 & 11.22 & 13.42 & 13.96 \\
SHARQ & \textbf{9.87} & \textbf{9.68} & \textbf{10.41} & \textbf{11.72} & \textbf{11.23} & \textbf{13.84} & 15.69 & \textbf{16.56} & \textbf{8.68} & \textbf{9.49} & \textbf{10.23} & \textbf{10.94} & \textbf{9.67} & \textbf{9.76} & \textbf{10.75} & \textbf{11.34} \\
\hlinewd{1.5pt}
\end{tabular}\hspace{5em}}
\label{tab:mape}
\end{table*}

\subsection{Simulation Experiments}

We first demonstrate that quantile loss can handle various kinds of error distributions and thus provide more stable and accurate uncertainty estimation than methods under Gaussian error assumption. We trained vanilla RNN models on three different sequential data with distinct error distributions. We implemented a model that has multiple quantile estimators with shared features, which enables more efficient training. The bagging method \citep{oliveira2014ensembles} is used as a baseline where we utilize model ensembles to produce confidence intervals. Figure \ref{fig:sim_plot} shows the advantage of quantile estimators on simulated sequential data, and Table \ref{tab:sim_res} compares forecasting results as well as demonstrates our model structure. Although it is difficult to capture the trend of discontinuous functions in Figure \ref{fig:sim_plot} (b) and (c), the quantile estimators are accurate and stable under both skewed and symmetric error distributions, where it also outperforms the baseline for all types of error distributions.

\subsection{Hierarchical Time Series}
We validate the performance of SHARQ on multiple real-world hierarchical time-series datasets, which include Australian Labour, FTSE \citep{doherty2005hierarchical}, M5 competition, and Wikipedia webpage views dataset (see Appendix \ref{sec:data} for details). This type of data usually contains categorical features (e.g., locations, genders) that can be used to aggregate across time series to construct hierarchical structures. We compare our method with state-of-the-art reconciliation algorithms MinT \citep{wickramasuriya2019optimal} and ERM \citep{ben2019regularized}, along with other baselines, including bottom-up (BU) and base forecast. To have a fair comparison, we first pre-process each dataset using information from categorical features. The bottom-up training procedure in Algorithm \ref{alg:bu} is then used for each method except for BU. Specifically, the model training settings of the base forecast, MinT and ERM are by default the same as SHARQ, except that they do not have mean and quantile reconciliation. As for MinT and ERM, extra reconciliations are performed after model training. In this case, the algorithm has access to the hierarchical information about the dataset. We also incorporate different time series forecasting algorithms into our framework, which ranges from linear auto-regressive model and RNN-GRU \citep{chung2014empirical} to advanced models such as LSTNet \citep{lai2018modeling} and N-Beats \citep{oreshkin2019n}. Although these models are not originally designed for hierarchical time series problems, we show that the performance on this task can be improved under our framework. 

Table \ref{tab:mape} and \ref{tab:crps} shows forecasting results across all reconciliation methods and models on Australian Labour (upper) and M5 (lower) dataset, the results are averaged across 3 runs. Specifically, MAPE \citep{makridakis2000m3} measures accuracy for point forecast by Eq.(\ref{contstrained_loss}), and $Continuous ~Ranked ~Probability ~Score$ (CRPS) \citep{matheson1976scoring} measures the holistic accuracy of a probabilistic forecast, using multiple quantiles. Overall, SHARQ outperforms other reconciliation baselines, resulting in much lower MAPE and CRPS over all four models, particularly at the higher aggregation levels. Specifically, although the bottom-up training of SHARQ leads to the same bottom level performance as BU and Base method, the error accumulation and inconsistency across the hierarchy leads to higher error in other aggregation levels. More importantly, the better performance of SHARQ over Base and BU in multiple datasets validates the necessity of hierarchical construction in DNN training. Besides, comparing the autoregressive model results with others, SHARQ tends to perform better when the forecasting model is less parsimonious for the dataset. Figure \ref{fig:eight_fig} presents multi-step forecasting results, which possess the advantage of coherent estimation at multiple quantile levels. 

\begin{figure*}[t!]
    \begin{minipage}{\textwidth}
    \centering
    \begin{tabular}{@{\hspace{-2.4ex}} c @{\hspace{-2.4ex}} @{\hspace{-2.4ex}} c @{\hspace{-2.4ex}} @{\hspace{-2.4ex}} c @{\hspace{-2.4ex}} @{\hspace{-2.4ex}} c @{\hspace{-2.4ex}}}
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/labour_forecast.png}
        %\vspace{-5pt}
        \\
        {\small{(a) Labour (SHARQ)}}
        \end{tabular} &
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/sim_small_forecast.png}
        %\vspace{-5pt}
        \\
        {\small{(b) FTSE (SHARQ)}}
        \end{tabular} & 
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/sales_forecast.png} 
        %\vspace{-5pt}
        \\
        {\small{(c) M5 (SHARQ)}}
        \end{tabular} &
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/wiki_forecast.png}
        %\vspace{-5pt}
        \\
        {\small{(d) Wiki (SHARQ)}}
        \end{tabular} \\
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/labour_forecast_mint.png}
        %\vspace{-5pt}
        \\
        {\small{(a) Labour (MinT-shr)}}
        \end{tabular} &
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/sim_small_forecast_mint.png}
        %\vspace{-5pt}
        \\
        {\small{(b) FTSE (MinT-ols)}}
        \end{tabular} & 
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/sales_forecast_mint.png} 
        %\vspace{-5pt}
        \\
        {\small{(c) M5 (MinT-shr)}}
        \end{tabular} &
        \begin{tabular}{c}
        \includegraphics[width=.276\textwidth]{images/wiki_forecast_mint.png}
        %\vspace{-5pt}
        \\
        {\small{(d) Wiki (MinT-sam)}}
        \end{tabular} \\
        \end{tabular}
    \end{minipage}
    \caption{Top and bottom level forecasts on four datasets using the LSTNet skip connection model. For each dataset, we plot the results of SHARQ and the second-best reconciliation method. P5 and P95 forecasts are the lower and upper boundaries of the forecast band. We use mean as the point estimator (also complement of P50) for all bottom-level data and other aggregation levels of Australian Labour and FTSE data.}
    \label{fig:eight_fig}
\end{figure*}

\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.2}
\scalebox{0.7}{
\begin{tabular}{c|cccc|cccc|cccc|cccc}
\hlinewd{1.5pt}
Algorithm & \multicolumn{4}{c}{ RNN } & \multicolumn{4}{c}{ Autoregressive } & \multicolumn{4}{c}{ LST-Skip } & \multicolumn{4}{c}{ N-Beats } \\
\hline
\multirow{2}{*}{ Reconciliation } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } & \multicolumn{4}{c}{ Level } \\
\hhline{|~|----|----|----|----|}
& 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 \\ \hline
BU & 0.244 & 0.221 & 0.186 & \textbf{0.149} & 0.401 & 0.367 & 0.303 & 0.231 & 0.241 & 0.222 & 0.193 & \textbf{0.142} & 0.232 & 0.211 & 0.196 & 0.154 \\
Base & 0.119 & 0.135 & 0.143 & \textbf{0.149} & 0.174 & 0.203 & 0.221 & 0.231 & 0.124 & 0.139 & 0.142 & \textbf{0.142} & 0.122 & 0.141 & 0.141 & 0.154 \\
MinT-sam & 0.106 & 0.135 & 0.139 & 0.152 & 0.167 & 0.191 & 0.214 & 0.227 & 0.106 & 0.125 & 0.133 & 0.156 & 0.106 & 0.119 & 0.141 & \textbf{0.153} \\
MinT-shr & 0.103 & 0.129 & 0.137 & 0.158 & 0.162 & 0.189 & 0.206 & 0.232 & 0.101 & 0.113 & 0.132 & 0.153 & 0.103 & \textbf{0.114} & 0.137 & 0.155 \\
MinT-ols & 0.109 & 0.133 & 0.142 & 0.159 & 0.167 & 0.194 & 0.215 & 0.233 & 0.109 & 0.124 & 0.133 & 0.154 & 0.111 & 0.123 & 0.142 & 0.155 \\
ERM & 0.126 & 0.147 & 0.152 & 0.156 & 0.164 & \textbf{0.178} & \textbf{0.192} & \textbf{0.201} & 0.132 & 0.145 & 0.149 & 0.162 & 0.121 & 0.138 & 0.143 & 0.158 \\
SHARQ & \textbf{0.097} & \textbf{0.124} & \textbf{0.133} & \textbf{0.149} & \textbf{0.157} & 0.187 & 0.199 & 0.231 & \textbf{0.089} & \textbf{0.096} & \textbf{0.126} & \textbf{0.142} & \textbf{0.092} & 0.115 & \textbf{0.136} & 0.154 \\ \hhline{|=|====|====|====|====|}
BU & 0.247 & 0.231 & 0.226 & \textbf{0.208} & 0.397 & 0.375 & 0.316 & 0.297 & 0.219 & 0.211 & 0.194 & \textbf{0.164} & 0.199 & 0.171 & 0.152 & \textbf{0.135} \\
Base & 0.162 & 0.167 & 0.193 & \textbf{0.208} & 0.231 & 0.257 & 0.265 & 0.297 & 0.146 & 0.152 & 0.175 & \textbf{0.164} & 0.079 & 0.128 & 0.136 & \textbf{0.135} \\
MinT-sam & 0.147 & 0.158 & 0.154 & 0.211 & 0.257 & 0.262 & 0.271 & 0.279 & 0.112 & 0.141 & 0.175 & 0.189 & 0.091 & 0.124 & 0.142 & 0.149 \\
MinT-shr & 0.134 & 0.142 & 0.146 & 0.213 & 0.256 & 0.248 & 0.268 & 0.288 & 0.096 & 0.137 & 0.134 & 0.171 & 0.083 & 0.112 & 0.147 & 0.166 \\
MinT-ols & 0.143 & 0.161 & 0.154 & 0.215 & 0.259 & 0.261 & 0.272 & 0.283 & 0.109 & 0.154 & 0.156 & 0.191 & 0.086 & 0.117 & 0.139 & 0.162 \\
ERM & 0.152 & 0.154 & 0.188 & 0.226 & 0.213 & 0.229 & \textbf{0.241} & \textbf{0.267} & 0.124 & 0.166 & 0.168 & 0.194 & 0.098 & 0.129 & 0.151 & 0.172 \\
SHARQ & \textbf{0.071} & \textbf{0.063} & \textbf{0.114} & \textbf{0.208} & \textbf{0.189} & \textbf{0.225} & 0.279 & 0.297 & \textbf{0.069} & \textbf{0.074} & \textbf{0.108} & \textbf{0.164} & \textbf{0.067} & \textbf{0.069} & \textbf{0.096} & \textbf{0.135} \\
\hlinewd{1.5pt}
\end{tabular}\hspace{5em}}
\caption{Performance measured by CRPS \citep{matheson1976scoring} on Australian Labour (755 time series), and M5 competition (42840 time series), lower values are better. Level 1 is the top aggregation level, and 4 is the bottom aggregation level.}
\label{tab:crps}
\end{table*}

\begin{figure}[h]
    \centering{
    \includegraphics[width=.48\textwidth]{images/coherency_plot.png}
    \caption{Coherency loss of SHARQ compared with the Base method on four datasets. Results are averaged across all the forecasting models.}}
    \label{fig:coherency}
\end{figure}

We pre-define the hyper-parameter $\lambda_i$ for vertex $v_i$ from Eq.(\ref{contstrained_loss}) level-wise, where we use the same $\lambda$s for all time series at the same level, and gradually decrease this value at higher aggregation levels. This is because time series at the same level possess similar magnitudes. With more vertices at lower levels, the chances of having consistency issues are higher, and error can accumulate to higher levels. 

We then evaluate the effect of regularization strength on forecasting coherency across the hierarchical structure; we summarize the result in Figure \ref{fig:coherency}, where the coherency loss drops dramatically after incorporating the hierarchical regularization at each level. Note that we mainly compare SHARQ with the Base method (SHARQ without regularization), as other reconciliation approaches generate absolute coherent results at the cost of sacrificing forecasting accuracy. More detailed evaluations can be found in Appendix \ref{sec:add_exp}.

\subsection{Comparison with Baseline Methods} 
Learning inter-level relationships through regularization helps SHARQ generalize better while mitigating coherency issues. It also provides a learnable trade-off between coherency and accuracy. From a computational perspective, MinT and ERM require one to compute matrix inversion explicitly. Note that the ERM method could compute the weight matrix on a validation set, but additional matrix computations are required during inference. Crucially, they depend on the Gaussian and unbiasedness assumptions, as stated in \citet{ben2019regularized, hyndman2011optimal, wickramasuriya2015forecasting} and their performance degrades noticeably when faced with actual data that do not match these assumptions well.


==> SHARQ-AISTATS21 (Version 7138)/tex/introduction.tex <==
\section{Introduction} \label{background}
\label{sec:intro}

\newcommand{\hy}{\hat{y}}
\newcommand{\hb}{\hat{\beta}}
\newcommand{\ty}{\Tilde{y}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\tY}{\Tilde{Y}}
\newcommand{\TL}{\widetilde{\mathcal{L}}_n}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\I}{\mathcal{I}}

\tikzstyle{circ} = [draw, circle, fill=white!20, radius=2.6, minimum size=.8cm, inner sep=0pt]
\tikzstyle{line} = [draw]

\begin{figure*}
\centering
{
\setlength{\tabcolsep}{1pt} 
\renewcommand{\arraystretch}{1} 
    \begin{tabu*}{cccc}
    \includegraphics[width=.26\textwidth]{images/us_region.pdf} & 
    \begin{tikzpicture}[node distance = 1.cm,auto]
    \node [circ] (step1) {$v_1$};
    \node [circ, below left = 0.3cm and 1.2cm of step1, label={793:{$e_{1, 2}$}}] (step2) {$v_2$};
    \node [circ, below right = 0.3cm and 1.2cm of step1, label={493:{$e_{1, 3}$}}] (step3) {$v_3$};
    \node [circ, below left = 0.3cm and 0.3cm of step2] (step4) {$v_4$};
    \node [circ, below right = 0.3cm and 0.3cm of step2] (step5) {$v_5$};
    \node [circ, below left = 0.3cm and 0.3cm of step3] (step6) {$v_6$};
    \node [circ, below right = 0.3cm and 0.3cm of step3] (step7) {$v_7$};
    \path [line, rounded corners] (step1) -| (step2);
    \path [line, rounded corners] (step1) -| (step3);
    \path [line, rounded corners] (step2) -| (step4);
    \path [line, rounded corners] (step2) -| (step5);
    \path [line, rounded corners] (step3) -| (step6);
    \path [line, rounded corners] (step3) -| (step7);
    \end{tikzpicture} &
    \includegraphics[width=.18\textwidth]{images/s_matrix.pdf} &
    \includegraphics[width=.18\textwidth]{images/hie_ts.png} \\
    (a) & (b) & (c) & (d) \\
    \end{tabu*}
    \caption{(a) Example of hierarchically related time series: state population growth forecast, the data is aggregated by geographical locations; (b) corresponding graph structure as nodes and vertices; (c) corresponding matrix representation with four bottom level time series and three aggregated levels; (d) time series forecast at each node.}}
    \label{fig:hierarchical_demo}
\end{figure*}


Hierarchical time series refers to a set of time series organized in a logical hierarchy with the parent-children relations, governed by a set of aggregation and disaggregation operations \citep{hyndman2011optimal, taieb2017coherent}. These aggregations and disaggregations can occur across multiple time series or over the same time series across multiple time granularities. An example of the first kind can be forecasting demand at county, city, state, and country levels \citep{hyndman2011optimal}. An example of the second kind of hierarchy is forecasting demand at different time granularities like daily, weekly, and monthly \citep{athanasopoulos2017forecasting}. The need to forecast multiple time series that are hierarchically related arise in many applications, from financial forecasting \citep{sasforecasting} to demand forecasting \citep{hyndman2016fast, zhao2016multi} and psephology \citep{lauderdale2019model}. The
recently announced M5 competition\footnote{https://mofc.unic.ac.cy/m5-competition/} from the International Institute of Forecasters also involves hierarchical forecasting on Walmart data with a \$100K prize. 
A novel challenge in such forecasting problems is to produce accurate forecasts while maintaining the consistency of the forecasts across multiple hierarchies. 


\paragraph{Related Works} Existing hierarchical forecasting methods predominantly employ linear auto-regressive (AR) models that are initially trained while ignoring the hierarchy. The output forecasts produced by these AR models are reconciled afterward for consistency. As shown in Figure \ref{fig:hierarchical_demo}(c), such reconciliation is achieved by defining a mapping matrix, often denoted by $S$, which encapsulates the mutual relationships among the time series \citep{hyndman2011optimal}. The reconciliation step involves inversion and multiplication of the $S$ matrix that leads to the computational complexity of  $\mathcal{O}(n^3 h)$, where $n$ is the number of nodes, and $h$ represents how many levels of hierarchy the set of time series are organized into. Thus,  reconciling hundreds of thousands of time series at a time required for specific industrial applications becomes difficult. Improved versions of the reconciliation were proposed by employing trace minimization \citep{wickramasuriya2015forecasting} and sparse matrix computation \citep{hyndman2016fast}. These algorithms assume that the individual base estimators are unbiased, which is unrealistic in many real-life applications. The unbiasedness assumption was relaxed in \citep{taieb2017coherent} while introducing other assumptions like ergodicity with exponentially decaying mixing coefficient. Moreover, all these existing methods try to impose any reconciliation constraints among the time series as a post inference step, which possesses two challenges: 1. ignoring the relationships across time series during training can potentially lead to suboptimal solutions, 2. additional computational complexity in the inference step, owing to the inversion of $S$ matrix, which makes it challenging to use the technique when a significant amount of time series are encountered in an industrial forecasting pipeline. 
%In our proposed method, we alleviate these shortcomings and also do not require the unbiasedness assumption on the individual estimators. 


A critical development in time series forecasting has been the application of Deep Neural Networks (DNN) \citep[e.g.,][]{chung2014empirical, lai2018modeling, mukherjee2018armdn, oreshkin2019n, salinas2019deepar, sen2019think, zhu2017deep} which have shown to outperform statistical auto-regressive or other statistical models in several situations. However, no existing method incorporates the hierarchical structure of the set of time series into the DNN learning step. Instead, one hopes that the DNN will learn the relationships from the data. Graph neural networks (GNN) \citep[e.g.,][]{franceschi2019learning, lachapelle2019gradient, wu2020connecting, yu2017spatio, yu2019dag, zhang2020deep, zheng2018dags} have also been used to learn inherent relations among multiple time series; however, they need a pre-defined graph model that can adequately capture the relationships among the time series.
Characterizing uncertainty of the DNN forecast is another critical aspect, which becomes even more complicated when additive noise does not follow a Gaussian distribution \citep[e.g.,][]{blundell2015weight, iwata2017improving, kuleshov2018accurate, lakshminarayanan2017simple, sun2019functional}. If the observation noise model is misspecified, then the performance would be poor however complex neural network architecture one uses. Other works like \citet{salinas2019deepar} use multiple observation noise models (Gaussian, Negative Binomial) and loss functions. It is left to human experts' discretion to select the appropriate loss based on the time series's nature. This approach cannot be generalized and involves human intervention; it is especially not feasible for an industrial forecasting pipeline where predictions are to be generated for a vast number of time series, which can have a widely varying nature of observation noise. Besides, Bayesian approaches also face problems as the prior distribution and loss function assumptions will not be met across all of the time series. One approach that does not need to specify a parametric form of distribution is through quantile regression. Prior works include combining sequence to sequence models with quantile loss to generate multi-step probabilistic forecasts \citep{wen2017multi} and modeling conditional quantile functions using regression splines \citep{gasthaus2019probabilistic}. These works are incapable of handling hierarchical structures within time series. 

Key aspects of multiple, related time series forecasting addressed by our proposed model include:
\begin{enumerate}
	\item introduction of a regularized loss function that captures the mutual relationships among each group of time series from adjacent aggregation levels,
	\item generation of probabilistic forecasts using quantile regression and simultaneously reconciling each quantile during model training,
	\item clear demonstration of superior model capabilities, especially on real e-commerce datasets with sparsity and skewed noise distributions.
\end{enumerate}
%In this paper, we further extend quantile regression into hierarchical time series forecasting framework by enabling each quantile to be coherent under the given structure.
%\textcolor{red}{quantile prior work on time series and quantile crossing here}
% A quantile based neural network was proposed in \cite{wen2017multi} to handle such non-parametric error distributions. In this paper, we present a general framework, named SHARQ  (Simultaneous HierArchically Reconciled Quantile regressions), for addressing the hierarchical forecasting problem. 
% In SHARQ, a suitable regularized loss incorporates the relationship among the time series and quantile loss is used to characterize the uncertainty in a non-parametric fashion.  A specific instance of SHARQ, wherein DNNs are used as the individual forecasters, is the Deep Quantile Hierarchical Forecasting Network (DQHFN).  

% The key contributions of this paper include:
% \begin{itemize}
% \item formulation of a generalized regularized loss function to incorporate the mutual relationships among subsets of time series,
% \item a method that avoids assuming that all  base forecasters are unbiased,
% \item an efficient method that simultaneous facilitates learning and reconciliation, and does not need a post-processing step that is typical of alternate methods 
% \item extending the Gaussian error model to general non-parametric distributions, 
% \item a distributed optimization formulation that avoids inverting a large matrix, making SHARQ scalable to large numbers of time series. 
% \end{itemize}
% The remainder of the paper is structured as follows: after a brief background, which also summarizes existing methods to forecast hierarchically related time series, we introduce  our proposed methodology in Section \ref{dqhfn}.  Section \ref{theory}  demonstrates the optimality of our method, discuss relevant statistical properties. Section \ref{experimental_results} presents several experimental results.

\paragraph{Background: Hierarchical Time Series Forecast}  Denote $b_t \in \mathbb{R}^m$, $a_t \in \mathbb{R}^k$ as the observations at time $t$ for the $m$ and $k$ series at the bottom and aggregation level(s), respectively. Then $y_t = S b_t \in \mathbb{R}^n$ contains observations at time $t$ for all levels. Similarly, let $\hat{b}_T(h)$ be the $h-$step ahead forecast on the bottom-level at time $T$, we can obtain forecasts in higher aggregation levels by computing $\hy_T(h) = S \hat{b}_T(h)$. This simple method is called bottom-up (BU), which guarantees reconciled forecasts. However, the error from bottom-level forecasts will accumulate to higher levels, leading to poor results. BU also cannot leverage any training data that is available at the more granular levels. A more straightforward approach called base forecast is to perform forecasting for each time series independently without considering the structure at all, i.e., compute $\hy_T(h) = \left[\hat{a}_T (h)^{\top} ~~ \hat{b}_T(h)^{\top}\right]^{\top}$, but this will apparently lead to irreconciled forecasts. Therefore, imposing constraints to revise the base forecasts is a natural choice to accommodate the hierarchical relationships. More specifically, the goal is to obtain some appropriately selected matrix $P \in \mathbb{R}^{m \times n}$ to combine the base forecasts linearly: $\ty_T(h) = SP\hy_T(h)$, where $\ty_T(h)$ is the reconciled forecasts which are now coherent by construction. The role of $P$ is to map the base forecasts into the forecasts at the most disaggregated level and sum them up by $S$ to get the reconciled forecasts. The previously mentioned approach \citep{ben2019regularized, hyndman2011optimal, hyndman2016fast, wickramasuriya2015forecasting} involves computing the optimal $P$ under different situations. A more detailed introduction can be found in Appendix \ref{sec:background}.

==> SHARQ-AISTATS21 (Version 7138)/tex/mainmethod.tex <==
\section{Simultaneous Hierarchically Reconciled Quantile Forecasting} \label{dqhfn}
We propose a new method for hierarchical time-series forecasts. Our approach fundamentally differs from others in that we move the reconciliation into the training stage by enabling the model to simultaneously learn the time series data from adjacent aggregation levels, while also integrating quantile regression to provide coherent forecasts for uncertainty bounds. We call our method Simultaneous HierArchically Reconciled Quantile Regression (SHARQ) to highlight these properties.

\subsection{Problem Formulation} \label{problem_formulation}

\paragraph{Graph Structure} Figure \ref{fig:hierarchical_demo}(b) shows a hierarchical graph structure where each node represents a time series, which is to be predicted over a horizon. The graph structure is represented by $ \{ V, E \}$, where $V := \{v_1, v_2, \dots, v_n \} $ are the vertices of the graph and $E := \{ e_{i_1, j_1}, e_{i_2, j_2}, \dots, e_{i_p, j_p} \}$ are the set of edges. Also, $e_{i, j} \in \{-1, 1\}$ is a signed edge where $i$ is the parent vertex and $j$ is the child. An example of the negative-signed edge can be forecasting surplus production, which is the difference between production and demand. The time series for vertex $i$ at time $t$ is represented as $x_{v_i} (t)$. For sake of simplicity, we assume the value of a time series at a parent level will be the (signed)  sum of the children vertices. 
This constraint relationship can be represented as $x_{v_i} (t) = \sum_{e_{i, k} \in E} e_{i, k} ~ x_{v_k} (t).$ We can later extend these to set of non-linear constraints: $x_{v_i} (t) =H_{v_i} \left(  \sum_{e_{i, k} \in E} e_{i, k} ~ x_{v_k} (t) \right)$, where $ H_{v_i} \in \mathbb{C}^1$. But linear hierarchical aggregation has already covered most real-world applications. The graph has hierarchies $L := \{ l_1, l_2, \dots, l_i, \dots, l_q\}$, where $l_i$ is the set of all vertices belonging to the $i^{th}$ level of hierarchy. Note that the graph representation using $\{ V, E \}$ is equivalent to the $S$ matrix in defining a hierarchical structure.

\tikzstyle{circ} = [draw, circle, fill=white!20, radius=2.6, minimum size=.8cm, inner sep=0pt]
\tikzstyle{line} = [draw]

% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     \begin{tikzpicture}[node distance = 1.2cm,auto]
%     \node [circ] (step1) {$v_1$};
%     \node [circ, below left = 0.3cm and 1.2cm of step1, label={793:{$e_{1, 2}$}}] (step2) {$v_2$};
%     \node [circ, below right = 0.3cm and 1.2cm of step1, label={493:{$e_{1, 3}$}}] (step3) {$v_3$};
%     \node [circ, below left = 0.3cm and 0.3cm of step2] (step4) {$v_4$};
%     \node [circ, below right = 0.3cm and 0.3cm of step2] (step5) {$v_5$};
%     \node [circ, below left = 0.3cm and 0.3cm of step3] (step6) {$v_6$};
%     \node [circ, below right = 0.3cm and 0.3cm of step3] (step7) {$v_7$};
%     \path [line, rounded corners] (step1) -| (step2);
%     \path [line, rounded corners] (step1) -| (step3);
%     \path [line, rounded corners] (step2) -| (step4);
%     \path [line, rounded corners] (step2) -| (step5);
%     \path [line, rounded corners] (step3) -| (step6);
%     \path [line, rounded corners] (step3) -| (step7);
%     \end{tikzpicture}
%     \caption{Hierarchical graph structure as nodes and vertices.}
%     \label{fig_hier}
% \end{wrapfigure}

\paragraph{Data Fit Loss Function}
We now formulate the learning problem for each node. Let $\{ x_{v_i} (t) ~|~ t = 0, \dots, T \}$ be the training data for vertex $v_i$, $w$ be the window of the auto-regressive features, and $h$ be horizon of forecast. Based on the window, we can create a sample of training data in the time stamp $m$ as: 
\begin{align*}
    \{ (X_m^i, Y_m^i) ~|~ X_m^i & = [ F \left ( x_{v_i} (m), \dots, x_{v_i} (m - w + 1) \right ) ], \\
    Y_m^i & = [x_{v_i} (m + 1), \dots, x_{v_i} (m + h)]  \}, \notag
\end{align*}
where $F \colon \mathbb{R}^{w+1} \to \mathbb{R}^{n_f}$ is the featurization function, which will generate a set of features; $n_f$ is the size of feature space, $h$ is the horizon of the forecast. It can be noted that $n_f \geq \omega$. In this fashion, we transform the forecasting problem to a regression one, where $n_f$ and $h$ capture the size of the feature space and the response. For instance, we can create a set of features for an ARIMA$(p, d, q)$ model based on the standard parameterization, where auto-regressive window size $w=p$ and the other features corresponding to the $d, q$ parameters will form the rest of the features.

We represent a forecasting model that learns the mean as a point estimate. Denote function $g_i : \mathbb{R}^{n_f} \times \mathbb{R}^{n_\theta} \to \mathbb{R}^{d}$, where $n_\theta$ represents the number of model parameters which are represented as $\theta_i \in \mathbb{R}^{n_\theta}$. The estimate from the model for $X_m^i$ will be $\hat{Y}_m^i := g_i (X_m^i, \theta_i)$. We can define a loss function for the $m^{th}$ sample at the $i^{th}$ vertex as $\L (\hat{Y}_m^i, ~ Y_m^i) = \L (g_i (X_m^i, \theta_i), ~ Y_m^i)$. We would assume the noise in training samples are of \texttt{i.i.d.} nature. As a consequence, the loss for the entire training data will be sum for each sample, i.e., $\sum_m \L (g_i (X_m^i, \theta_i), Y_m^i)$. Noted that this formulation will work for neural networks or ARIMA but not for Gaussian Processes, where we need to model the covariance of the uncertainties across the samples.

\paragraph{Reconciled Point Forecast}
We then describe how to incorporate reconciliation constraints into the loss functions for the vertices. The constraints at different levels of hierarchy will have different weights, which we denote as a function $w_c: L \to \mathbb{R}$. We define another function that maps any vertex to the hierarchy level, $LM: V \to L$. For any vertex $v_i$, the corresponding weight for the constraint is given by  $ \lambda_{v_i} := w_c \circ LM (v_i)$. The constrained loss for vertex $v_i$ will be 
\begin{align} 
& \L_c (g_i (X_m^i, \theta_i), Y_m^i, g_k (X_m^k, \theta_k)) := \L (g_i (X_m^i, \theta_i), Y_m^i) \nonumber \\
& + \lambda_i \parallel g_i (X_m^i, \theta_i) - \sum_{e_{i, k} \in E} \left ( e_{i, k} ~g_k (X_m^k, \theta_k) \right ) \parallel^2 .
\label{contstrained_loss}
\end{align}  
Note that the data fit loss and the reconciliation, as described thus far, are catered to the point estimate of the mean forecasts.

\subsection{Reconciling Probabilistic Forecast using Quantiles} \label{sec_qloss}
% For a wide ranging applications, probabilistic forecasts need to be generated over a range of time. Most notably, \cite{hyndman2011optimal} and \cite{wickramasuriya2015forecasting} assume that the uncertainty or error distribution at every future point of time can be represented as Gaussians. This is not a reasonable assumption, as for many forecasting problems, the errors are better modelled by other distributions e.g. Negative Binomial, Poisson, Cauchy and even distributions that are difficult to  parametrically specify. In such cases, using a Gaussian assumption will lead to mis-specification of the uncertainty bounds. Also, it can become cumbersome to modify the loss function based on an increasing number of distributions. Recently, \cite{wen2017multi} proposed a new approach by using quantile loss, which allows one to model the error distribution in a non-parametric fashion. The estimator (e.g. linear auto-regressor or neural network) will aim at minimizing a loss directly represented in terms of the quantiles. We could achieve this by fitting two quantile regressors to obtain estimates of upper and lower bounds for prediction intervals, then add regularization to the boundaries to make sure they are consistent with the hierarchies.
Generating probabilistic forecasts over a range of time is significant for wide-ranging applications. Real-world time series data is usually sparse and not uniformly sampled. It is unreasonable to assume that the uncertainty or error distribution at every future point of time as Gaussians. A standard approach to solve this problem is using quantile loss, which allows one to model the error distribution in a non-parametric fashion. The estimator will aim at minimizing a loss directly represented in terms of the quantiles. Simultaneously, quantile can be used to construct confidence intervals by fitting multiple quantile regressors to obtain estimates of upper and lower bounds for prediction intervals. The quantile loss $\rho_{\tau} (y)$ is defined as
$\rho_{\tau} (y, ~ Q_{\tau}) = \left( y - Q_{\tau} \right). (\tau - \mathbb{I}_{(y<Q_{\tau})}),$
where $Q_{\tau}$ is the $\tau^{th}$ quantile output by an estimator. We will adopt quantiles in our framework, and pre-specified quantile ranges will represent the forecasting distribution. For simplicity, we denote $Q_i^{\tau} = Q^{\tau}_i (X_m^i, \theta_i)$ as the $\tau^{th}$ quantile estimator for node $i$. Eq.(\ref{quantile}) demonstrates a quantile version of the probabilistic estimator; it aims to produce multiple forecasts at different quantiles while maintaining a coherent median forecast which will be used to reconcile other quantiles:
\begin{align}
     & \L_c (Q_i, Y_m^i, Q_k) := \nonumber \\
     & \sum_{\tau = \tau_0}^{\tau_q}\rho_{\tau} (Q^{\tau}_i, Y_m^i) %\nonumber \\
 + \lambda_i  \parallel Q^{50}_i - \sum_{e_{i, k} \in E} e_{i, k}  Q^{50}_i \parallel^2,
\label{quantile}
\end{align}
where $[\tau_0, \dots, \tau_q]$ are a set of quantile levels, and $Q_i = [Q^{\tau_0}_i, \dots, Q^{\tau_q}_i]$. To further guarantee that estimation at each quantile is coherent across the hierarchy, the straightforward solution is to add consistency regularization for each quantile like Eq.(\ref{quantile}). However, too many regularization terms would not only increase the number of hyper-parameters, but also complicate the loss function, where the result may even be worse as it is hard to find a solution to balance each objective. Moreover, a quantile estimator does not hold the additive property. As an example, assume $X_1 \sim N(\mu_1, \sigma_1^2)$, $X_2 \sim N(\mu_2, \sigma_2^2)$ are independent random variables, and define $Y = X_1 + X_2$. Then $Q_{Y}^{\tau} = Q_{X_1}^{\tau} + Q_{X_2}^{\tau}$ is true only if $X_1 = C \times X_2$, where $C$ is arbitrary constant. This requirement cannot be satisfied. But for any $\tau$, we have $(Q_{Y}^{\tau} - \mu_Y )^2 = (Q_{X_1}^{\tau} - \mu_{X_1})^2 + (Q_{X_2}^{\tau} - \mu_{X_2})^2$, the proof of above properties can be found in Appendix \ref{sec:nonadd}. Given these properties, we can formulate a new objective to make an arbitrary quantile consistent:
\begin{align}
    & \L_q (Q_i, Y_m^i, Q_k) := \label{quantile_recon} \\
    & \left [f\left(Q^{\tau}_i - Q^{50}_i\right) 
 	 - \sum_{e_{i, k} \in E} e_{i, k} ~ f\left(Q^{\tau}_k - Q^{50}_k\right) + \mathrm{Var}(\epsilon)\right ]^2, \nonumber
\end{align}
where $\epsilon$ is the mean forecast's inconsistency error, which is mostly a much smaller term for a non-sparse dataset, and $f$ is the distance metric. Eq.(\ref{quantile_recon}) is zero when $f$ is a squared function and the given data satisfies \texttt{i.i.d.} Gaussian assumption. Therefore,  optimizing Eq.(\ref{quantile_recon}) ``forces'' this additive property in non-Gaussian cases and is equivalent to reconcile the quantile estimators, which can also be interpreted as reconciliation over the variance across adjacent aggregation levels. Empirically, this approach calibrates multiple quantile predictions to be coherent and mitigates the quantile crossing issue \citep{liu2009stepwise}.
% We will empirically verify the advantage of this approach in later section. \textcolor{red}{replace median into the reconciled mean estimator trained, this is median under gaussian assumption, but also make sure each quantile does not deviate too much from the mean for non-symmetric error, also change the L2 loss to general functions, also add quantile crossing discussion}

\begin{algorithm}[t]
\small
\caption{SHARQ}
\label{alg:bu}
\begin{algorithmic}
\STATE \textbf{Input}:~~Training data $\mathcal{I}_1 = \{X_i, Y_i\}_{i=1}^{T_1}$, testing data $\mathcal{I}_2 = \{X_i, Y_i\}_{i=1}^{T_2}$.
\STATE \textbf{Process}:
\STATE train each leaf node (e.g., $v_4$ to $v_7$ in Figure \ref{fig:hierarchical_demo}(b)) independently without regularization
\FOR{each vertex $v$ at upper level $l$ (e.g., $l = 2$ for $v_3$, $v_2$, then $l = 1$ for $v_1$)}
\STATE train vertex $v$ at level $l$ using Eq.(\ref{quantile})
\ENDFOR
\STATE Reconciled Median Forecast \textbf{MF} $\leftarrow$ \textbf{Models}($\mathcal{I}_2$)
\FOR{each vertex $v$ at upper level $l$}
\STATE train vertex $v$ at level $l$ using Eq.(\ref{quantile_recon}) and \textbf{MF}
\ENDFOR
\STATE \textbf{Output}: ~ Reconciled forecasts at pre-specified quantiles.
\end{algorithmic}
\end{algorithm}

\subsection{SHARQ Algorithm}
Our formulation can be combined with a bottom-up training approach to reconciling forecasts for each quantile simultaneously. Since the time series at the leaf (disaggregated) level are independent of higher aggregation levels, we can use the lower-level forecasting results to progressively reconcile the forecasting models at higher levels without revisiting previous reconciliations, till the root is reached. In contrast, if top-down training is applied, one needs to reconcile both higher (previously visited) and lower-level data at an intermediate vertex, since other time series at that intermediate level may have changed. Algorithm \ref{alg:bu} describes our procedure. We now address the remaining aspects.

\paragraph{Beyond Gaussian Noise Assumption.} Noise distributions for many real-world datasets (e.g., e-commerce data) are heavily skewed, so a Gaussian model may not be appropriate. For multi-level time series, data at the most disaggregated (lowest) level is more likely to be sparse, which makes the quantile reconciliation in Eq.(\ref{quantile_recon}) less accurate. In such situations, one can substitute median with the mean estimator as in Eq.(\ref{contstrained_loss}) for training lower-level time series. One can also mix-and-match between mean and median estimators at higher aggregation levels depending on the data characteristics. Finding a suitable function $f$ for quantile reconciliation as in Eq.(\ref{quantile_recon}) is an alternative way to tackle  non-symmetric errors \citep{li20081}. 
    
\paragraph{Efficient Training and Inference} SHARQ is time and memory efficient, scaling well in both aspects with large datasets. One can simultaneously train multiple time series and keep a running sum for reconciliation. Since coherent probabilistic forecasts are enforced during training, no extra post-processing time is needed (see Appendix \ref{sec:add_exp} for details). Besides, SHARQ does not force one to use deep forecasting models or to use the same type of model at each node; in fact, any model where gradient-based optimization can be used is allowable, and one can also mix-and-match. For cases where the time series at a given level are structurally very similar \citep{zhu2017deep}, they can be grouped (e.g., by clustering), and a single model can be learned for the entire group.

%\paragraph{Data Aggregation} 

%\textcolor{red}{talk about running summation and how to efficiently get result to avoid memory issue, see computation time in supplementary material. also issues of insufficient data at top level; mix and match, quantile estimator and point estimators according to the dataset property}

%\subsection{General Data Aggregation} add stuff here


